Testing the Higgs Boson Coupling to Gluons

We study the possibility to separate in gluon fusion loop-induced Higgs boson production from point-like production. The Higgs boson is reconstructed in the Hgg final state at very large transverse momentum. Using the Higgs boson yields (normalized to the overall rate) and the shape of the Higgs boson pt distribution the two hypotheses can be separated with 2 standard deviations with an integrated luminosity of about 500 fb^-1. The largest experimental uncertainty affecting this estimate is the background event yield. The theoretical uncertainties from missing top mass effects are large, but can be decreased with dedicated calculations.

==> symbols.tex <==
\RequirePackage{xspace}


\def\hgg    {\ensuremath{H \to \gamma\gamma}}

\def\Emax   {\ensuremath{E_{\mathrm{max}}}}
\def\rmm         {\ensuremath{\Delta R(\mu\mu)}}
\def\ptmuone     {\ensuremath{\pt_{\mu,1}}}
\def\ptmutwo     {\ensuremath{\pt_{\mu,2}}}
\def\ptb         {\ensuremath{\pt_{B}}}
\def\pth         {\ensuremath{\pt_{H}}}
\def\ptg         {\ensuremath{\pt_{\gamma}}}
\def\ptgg        {\ensuremath{\pt_{\gamma\gamma}}}
\def\mgg        {\ensuremath{m_{\gamma\gamma}}}
\def\etamuone    {\ensuremath{\eta_{\mu,1}}}
\def\etamutwo    {\ensuremath{\eta_{\mu,2}}}
\def\etab        {\ensuremath{\eta_{B}}}
\def\pvw         {\ensuremath{\langle w\rangle}}
\def\fl          {\ensuremath{\ell_{3D}}}
\def\flxy        {\ensuremath{\ell_{xy}}}
\def\fls         {\ensuremath{\ell_{3D}/\sigma(\ell_{3D})}}
\def\flsxy       {\ensuremath{\ell_{xy}/\sigma(\ell_{xy})}}
\def\pa          {\ensuremath{\alpha_{3\mathrm{D}}}}
\def\chidof      {\ensuremath{\chi^2/\mathrm{dof}}}
\def\closetrk    {\ensuremath{N_{\mathrm{trk}}^{\mathrm{close}}}}
\def\closetrkA   {\ensuremath{N_{\mathrm{trk}}^{\mathrm{close}, 1\sigma}}}
\def\closetrkB   {\ensuremath{N_{\mathrm{trk}}^{\mathrm{close}, 2\sigma}}}
\def\closetrkC   {\ensuremath{N_{\mathrm{trk}}^{\mathrm{close}, 3\sigma}}}
\def\iso         {\ensuremath{I}}
\def\isomu       {\ensuremath{I_{\mu}}}
\def\isomuone    {\ensuremath{I_{\mu_1}}}
\def\isomutwo    {\ensuremath{I_{\mu_2}}}
\def\xpdistmu    {\ensuremath{d_{\mu}^{xp}}}
\def\xpdistmuone {\ensuremath{d_{\mu_1}^{xp}}}
\def\xpdistmutwo {\ensuremath{d_{\mu_2}^{xp}}}
\def\docatrk     {\ensuremath{d^{\mathrm{0}}_\mathrm{ca}}}
\def\dca         {\ensuremath{d_\mathrm{ca}}}
\def\ip          {\ensuremath{\delta_{3D}}}
\def\ips         {\ensuremath{\delta_{3D}/\sigma(\delta_{3D})}}
\def\lip         {\ensuremath{\ell_{z}}}
\def\lips        {\ensuremath{\ell_{z}/\sigma(\ell_{z})}}
\def\pvdchi      {\ensuremath{\Delta(\chi^2)}}
\def\othervtx    {\ensuremath{\Delta{\cal P}}}

\def\mll   {\ensuremath{m_{\mu\mu}}}
\def\dof   {\ensuremath\mathrm{dof}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Teaching
\def\ket#1        {\ensuremath|{#1}\rangle}
\def\bra#1        {\ensuremath\langle{#1}|}
\def\braket#1#2   {\ensuremath\langle{#1}|{#2}\rangle}
\def\tfi#1#2#3    {\ensuremath\langle{#1}|{#2}|{#3}\rangle}
\def\vtwo#1#2     {\ensuremath\left(\begin{array}{c}{#1}\\{#2}\end{array}\right)}
\def\vthree#1#2#3 {\ensuremath\left(\begin{array}{c}{#1}\\{#2}\\{#3}\end{array}\right)}
\def\me           {\ensuremath\mathcal{M}}
\def\ame          {\ensuremath|\mathcal{M}|^2}
\def\asme         {\ensuremath\overline{|\mathcal{M}|^2}}

\def\psib         {\ensuremath\overline{\psi}}

\newcommand{\mat}[2][cccccccccccccccccccccccccc]{\left(
   \begin{array}{#1} 
    #2\\
   \end{array}
  \right)
}
 
\def\vvA        {\ensuremath\left(\begin{matrix} 0 \\ 0 \end{matrix}\right)}
\def\vvB        {\ensuremath\left(\begin{matrix} 1 \\ 0 \end{matrix}\right)}
\def\vvC        {\ensuremath\left(\begin{matrix} 0 \\ 1 \end{matrix}\right)}
\def\vvD        {\ensuremath\left(\begin{matrix} 1 \\ 1 \end{matrix}\right)}

\def\vvvA        {\ensuremath\left(\begin{matrix} 0 \\ 0 \\ 0\end{matrix}\right)}
\def\vvvB        {\ensuremath\left(\begin{matrix} 1 \\ 0 \\ 0\end{matrix}\right)}
\def\vvvC        {\ensuremath\left(\begin{matrix} 0 \\ 1 \\ 0\end{matrix}\right)}
\def\vvvD        {\ensuremath\left(\begin{matrix} 0 \\ 0 \\ 1\end{matrix}\right)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Physics symbols
\def\cpt   {\ensuremath{C\kern-0.2em P\kern-0.1em T}}
\def\cp    {\ensuremath{C\kern-0.2em P}}
\def\cpv   {\ensuremath{C\kern-0.2em P\kern-1.0em / }}
\def\CPV   {\cp-violation}
\def\CPTV  {\cpt-violation}
\def\bfsx  {$B$-physics}
\def\ETm   {\ensuremath{E_T\kern-1.2em/\kern0.6em}}
\def\ET    {\ensuremath{E_T}}
\def\kT    {\ensuremath{k_T}}
\def\ptm   {\ensuremath{p_\perp\kern-1.1em/\kern0.5em}}
%\def\pvecm {\ensuremath{\vec{p} \kern-1.1em/\kern0.5em}}
\def\pvecm {\ensuremath{\vec{p} \kern-0.4em/\kern0.1em}}
\def\pvec  {\ensuremath{\vec{p}}}

\def\dsj   {\ensuremath{D_{sJ}}}
\def\vxb   {\ensuremath{|V_{xb}|}}
\def\vud   {\ensuremath{|V_{ud}|}}
\def\vus   {\ensuremath{|V_{us}|}}
\def\vub   {\ensuremath{|V_{ub}|}}
\def\vcd   {\ensuremath{|V_{cd}|}}
\def\vcs   {\ensuremath{|V_{cs}|}}
\def\vcb   {\ensuremath{|V_{cb}|}}
\def\vtd   {\ensuremath{|V_{td}|}}
\def\vts   {\ensuremath{|V_{ts}|}}
\def\vtb   {\ensuremath{|V_{tb}|}}

\def\deltam{\ensuremath{\delta m}}
\def\dm    {\ensuremath{\Delta m}}
\def\dt    {\ensuremath{\Delta t}}
\def\dg    {\ensuremath{\Delta \gamma}}
\def\dG    {\ensuremath{\Delta \Gamma}}
\def\dmt   {\ensuremath{\Delta mt}}
\def\dmdt  {\ensuremath{\Delta m \Delta t}}
\def\dms   {\ensuremath{\Delta m_s}}
\def\dmst {\ensuremath{\Delta m_s t}}
\def\dmm   {\ensuremath{\Delta m^2}}
\def\TBY   {\ensuremath{\theta_{\Bz, D^*\ell}}}

\def\de    {\ensuremath{\Delta E}}
\def\mes   {\ensuremath{m_{ES}}}

\def\msd{\ensuremath{\overline{m}_D^2}}
\def\lbar{\ensuremath{\overline{\Lambda}}}
\def\lone{\ensuremath{\lambda_1}}
\def\ltwo{\ensuremath{\lambda_2}}

\def\MUP   {\ensuremath{\mu_\pi^2}}
\def\MUG   {\ensuremath{\mu_G^2}}
\def\RHOD  {\ensuremath{\rho_D^3}}
\def\RHOLS {\ensuremath{\rho_{LS}^3}}


\def\cd {\ensuremath{{\cal D}}}
\def\cbf {\ensuremath{{\cal B}}}
\def\clu {\ensuremath{{\cal L}}}
\def\cor {\ensuremath{{\cal O}}}
\def\adg {\ensuremath{{\cal A}_{\Delta\Gamma}}}

% -- b->ulnu analysis
\def\mmiss{\ensuremath{{m_{miss}^2}}}
%%\def\rusl{\ensuremath{{R_{u/sl}}}}
\def\rusl{\ensuremath{{R_{u}}}}
\def\mh{\ensuremath{{m_{had}}}}
\def\mmxx {\ensuremath{\langle m_X^2 \rangle~}}
\def\mmx {\ensuremath{\langle m_X \rangle~}}
\def\mxqq{\ensuremath{(m_X, Q^2)}}
\def\mX{\ensuremath{{m_X}}}
\def\mx{\ensuremath{{m_X}}}
\def\mxcut{\ensuremath{{m_X^{cut}}}}
\def\pstar{\ensuremath{{p^*}}}
\def\qtot{\ensuremath{{Q_{tot}}}}
\def\pt{\ensuremath{{p_\perp}}}
\def\mt{\ensuremath{{m_\perp}}}

\def\pslash{\ensuremath{{p\kern-0.45em /}}}
\def\pvecslash{\ensuremath{{\vec{p} \kern-0.45em /}}}

% -- Hadronic moments
\def\meanmxx   {\ensuremath{\langle m_X^2 \rangle}}
\def\meanmx    {\ensuremath{\langle m_{X} \rangle}}
\def\mean#1    {\ensuremath{\langle #1 \rangle}}

% -- Processes
\def\Bpilnu    {\ensuremath{\Bb\to \pi\ell\nub}}
\def\Bmpilnu   {\ensuremath{\Bm\to \pi^0\ell^-\nub}}
\def\Betalnu   {\ensuremath{\Bb\to \eta\ell\nub}}
\def\Brholnu   {\ensuremath{\Bb\to \rho\ell\nub}}
\def\Bmrholnu  {\ensuremath{\Bb\to \rho^0\ell^-\nub}}
\def\Bomegalnu {\ensuremath{\Bb\to \omega\ell\nub}}
\def\Brhoenu   {\ensuremath{\Bb\to \rho e\nub}}
\def\Bzrhoenu  {\ensuremath{\Bz\to \rho^- e^+\nub}}

\def\Bdlnu     {\ensuremath{\Bb\to D\ell\nub}}
%%\def\Bdstarlnu {\ensuremath{B\to \Dstarb \ell^+ \nu}}
\def\Bdstarlnu {\ensuremath{\Bb\to \Dstar \ell \nub}}
\def\Bzdstarlnu {\ensuremath{\Bzb\to \Dstarp \ell^- \nub}}
\def\Bzdstarenu {\ensuremath{\Bzb\to \Dstarp e^- \nub}}

\def\bll     {\ensuremath{\Bz\to \ell^+\ell^-}}
\def\bee     {\ensuremath{\Bz\to e^+e^-}}
\def\bmm     {\ensuremath{B\to \mu^+\mu^-}}
\def\bem     {\ensuremath{\Bz\to e^\pm\mu^\mp}}
\def\btt     {\ensuremath{\B\to \tau^+\tau^-}}
\def\bdtt     {\ensuremath{\Bz\to \tau^+\tau^-}}
\def\bstt     {\ensuremath{\Bs\to \tau^+\tau^-}}
\def\bsmt     {\ensuremath{\B\to \mu^\pm\tau^\mp}}
\def\bmt     {\ensuremath{\B\to \mu^\pm\tau^\mp}}
\def\bmn     {\ensuremath{B^+\to \mu^+\nu_\mu}}
\def\btn     {\ensuremath{B^+\to \tau^+\nu_\tau}}
\def\bln     {\ensuremath{B^+\to \ell^+\nu_\ell}}
\def\bgen    {\ensuremath{B^-\to \gamma e\nub}}
\def\bgee    {\ensuremath{B^-\to \gamma e^+e^-}}
\def\bgg     {\ensuremath{B^-\to \gamma \gamma}}

\def\jpsitomu {\ensuremath{\jpsi\to \mu^+\mu^-}}
\def\bdmm     {\ensuremath{B^0\to  \mu^+\mu^-}}
\def\bdpipi   {\ensuremath{B^0\to  \pip\pim}}
\def\bdpik    {\ensuremath{B^0\to  \Kp\pim}}
\def\bdpimunu {\ensuremath{B^0\to  \pim\mup\nu}}
\def\bdmumupz {\ensuremath{B^0\to  \mup\mun\piz}}
\def\lbppi    {\ensuremath{\Lambda_b\to \pim p}}
\def\lbpk     {\ensuremath{\Lambda_b\to K^- p}}
\def\butrmunu {\ensuremath{B^+\to \mup\mun\mup \nu}}
\def\bctrmunu {\ensuremath{B_c\to \mup\mun\mup \nu}}
\def\bcpsimunu{\ensuremath{B_c\to \jpsi(\to\mup\mun)\mup \nu}}

\def\bdmm     {\ensuremath{B^0  \to \mu^+\mu^-}}
\def\bsmm     {\ensuremath{B^0_s\to \mu^+\mu^-}}
\def\bskk     {\ensuremath{B^0_s\to K^+K^-}}
\def\bspipi   {\ensuremath{B^0_s\to \pip\pim}}
\def\bspik    {\ensuremath{B^0_s\to K^-\pip}}
\def\bdkk     {\ensuremath{B^0\to K^+K^-}}
\def\bdpipi   {\ensuremath{B^0\to \pip\pim}}
\def\bdpik    {\ensuremath{B^0\to K^-\pip}}
\def\bskmunu  {\ensuremath{B^0_s\to K^-\mup\nu}}
\def\bsmumug  {\ensuremath{B^0_s\to \mup\mun\gamma}}
\def\bsmmg    {\ensuremath{B^0_s\to \mu^+\mu^-\gamma}}
\def\bdll     {\ensuremath{B^0\to \ell^+\ell^-}}
\def\bsll     {\ensuremath{B^0_s\to \ell^+\ell^-}}
\def\bstt     {\ensuremath{B^0_s\to \tau^+\tau^-}}
\def\bdmt     {\ensuremath{B^0  \to \mu^\pm\tau^\mp}}
\def\bsmt     {\ensuremath{B^0_s\to \mu^\pm\tau^\mp}}
\def\bsdmm    {\ensuremath{B^0_{s (d)}\to \mu^+\mu^-}}
\def\bsdll    {\ensuremath{B^0_{s (d)}\to \ell^+\ell^-}}
\def\bsdtt    {\ensuremath{B^0_{s (d)}\to \tau^+\tau^-}}
\def\tmmm     {\ensuremath{\tau\to \mu\mu\mu}}

\def\hbb      {\ensuremath{H\to \bbbar}}
\def\htt      {\ensuremath{H\to \taup\taum}}
\def\ttH      {\ensuremath{\ttbar H}}

\def\meg      {\ensuremath{\mu\to e\gamma}}
\def\meee     {\ensuremath{\mu\to eee}}
\def\pgg      {\ensuremath{\piz\to \g\g}}


\def\bsg     {\ensuremath{b\to s\gamma}}
\def\bulnu   {\ensuremath{b\to u\ell\nub}}
\def\bclnu   {\ensuremath{b\to c\ell\nub}}
\def\bcenu   {\ensuremath{b\to c e\nub}}
\def\bcmunu  {\ensuremath{b\to c \mu\nub}}
\def\buenu   {\ensuremath{b\to u e\nub}}

\def\bxlnu   {\ensuremath{b\to X\ell^-\nub}}
\def\Bxenu   {\ensuremath{\Bb\to Xe^-\nu}}

\newcommand {\Bxlnu}{\ensuremath{\Bb \rightarrow X \ell \bar{\nu}}}
\newcommand {\Bxclnu}{\ensuremath{\Bb \rightarrow X_c \ell \bar{\nu}}}
\newcommand {\Bxulnu}{\ensuremath{\Bb \rightarrow X_u \ell \bar{\nu}}}
\def\Bpxenu {\ensuremath{\Bp\to Xe^+\nu}}
\def\Bzxenu {\ensuremath{\Bz\to Xe^+\nu}}

\def\Bulnu   {\ensuremath{\Bb\to X_{u}\ell\nub}}
\def\Buenu   {\ensuremath{\Bb\to X_{u} e\nub}}
\def\Bclnu   {\ensuremath{\Bb\to X_{c}\ell\nub}}
\def\Bxulnu  {\ensuremath{\Bb\to X_{u}\ell\nub}}
\def\Bxuenu  {\ensuremath{\Bb\to X_{u} e\nub}}
\def\Bxclnu  {\ensuremath{\Bb\to X_{c}\ell\nub}}

\def\bfactory  {{{\sl B}-factory}}
\def\bfactories{{{\sl B}-factories}}
\def\bFactory  {{{\sl B}-Factory}}
\def\breco     {\ensuremath{B_{reco}}}
\def\btag      {\ensuremath{B_{tag}}}
\def\bdecay    {{$B$-decay}}
\def\bDecay    {{$B$-Decay}}
\def\bdecays   {{$B$-decays}}
\def\bDecays   {{$B$-Decays}}
\def\bhadron   {{$b$-hadron}}
\def\bhadrons  {{$B$-hadrons}}
\def\bmeson    {{$B$-meson}}
\def\bmesons   {{$B$-mesons}}
\def\bquark    {{$b$-quark}}
\def\bquarks   {{$b$-quarks}}
\def\bphysics  {{$b$-physics}}
\def\Bphysics  {{$B$-physics}}

% -- Abbreviations
\def\ie   {{\it i.e.}}
\def\cf   {{\it cf.}}
\def\eg   {{\it e.g.}}
\def\etal {{\it et~al.}}
\def\etc  {{\it etc.}}


% -- Gimmicks
\def\rtr    {{$\red\triangleright\black$}}
\def\barrow {{$\blue\to\black$}}
\def\bpoint {{$\blue\bullet\black$}}
\def\npoint {{\phantom{$ \blue\bullet\black$}}}

\newcommand\bfac   {$B$-Factories}


\newcommand\bu   {\ensuremath{b\to u}}
\newcommand\bc   {\ensuremath{b\to c}}

\newcommand\islbcd {inclusive semileptonic $B\to c\ell\nu$}
\newcommand\islbud {inclusive semileptonic $B\to u\ell\nu$}

% Quantities
\def\tg     {\ensuremath {\theta^{*}_T}}
\def\ctg     {\ensuremath {\cos{\tg}}}
\def\cth     {\ensuremath {\cos{\theta_{H}}}}
\def\cthe    {\ensuremath {\cos{\theta_{H\,\eta'}}}}
\def\cthr    {\ensuremath {\cos{\theta_{H\,\rho}}}}
\def\ctb     {\ensuremath {\cos{\theta^{*}_{B}}}}
\def\ebeam     {\ensuremath {E^{*}_{b}}}
\def\egcms     {\ensuremath {E^{*}_{\gamma}}}
\def\mkpi      {\ensuremath {M_{\Kp \pim}}}
%References
%\def\npb  #1 #2 #3 {Nucl.~Phys.~B~{\bf#1},\ #2 (#3)}
%\def\plb  #1 #2 #3 {Phys.~Lett.~B~{\bf#1},\ #2 (#3)}
%\def\pr   #1 #2 #3 {Phys.~Rep.~{\bf#1},\ #2 (#3)}
%\def\prd  #1 #2 #3 {Phys.~Rev.~D~{\bf#1},\ #2 (#3)}
%\def\prl  #1 #2 #3 {Phys.~Rev.~Lett.~{\bf#1},\ #2 (#3)}
%\def\RMP  #1 #2 #3 {Rev.~Mod.~Phys.~{\bf#1},\ #2 (#3)}
%\def\zpc  #1 #2 #3 {Z.~Phys.~C~{\bf#1},\ #2 (#3)}
%\def\rmp #1 #2 #3 {Rev.~Mod.~Phys~{\bf#1},\ #2 (#3)}
%\def\npbps #1 #2 #3 {Nucl.~Phys.~B.~proc.~suppl~{\bf#1},\ #2 (#3)}
%\def\progtp #1 #2 #3 {Prog.~Theo.~Phys~{\bf#1},\ #2 (#3)}
%\def\etal{{\it et al.}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\ellb        {\ensuremath{\bar{\ell}}\xspace}
\def\nub        {\ensuremath{\bar{\nu}}\xspace}
%\def\nub        {\kern 0.3em\overline{\kern -0.3em \nu\kern 0.3em}{}\xspace}
\def\nunub      {\ensuremath{\nu{\bar{\nu}}}\xspace}
\def\nunub      {\ensuremath{\nu{\bar{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\Qbar  {\ensuremath{\overline Q}\xspace}
\def\ffbar {\ensuremath{f\overline f}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\QQbar {\ensuremath{Q\overline Q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}
\def\pbar  {\ensuremath{\overline p}\xspace}
\def\ppbar {\ensuremath{p\overline p}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\bar{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\bar{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\bar{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\BsBsb   {\ensuremath{\Bs {\kern -0.16em \Bsb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bd      {\ensuremath{B^0_d}\xspace}
\def\Bs      {\ensuremath{B^0_s}\xspace}
\def\Bc      {\ensuremath{B^+_c}\xspace}
\def\Bsb     {\ensuremath{\Bzb_s}\xspace}
\def\Nz      {\ensuremath{M^0}\xspace}
\def\Nbar    {\kern 0.18em\bar{\kern -0.18em M}{}}
\def\Nzb     {\ensuremath{\Nbar^0}}
\def\NzNzb   {\ensuremath{\Nz {\kern -0.16em \Nzb}}}
\def\Nh      {\ensuremath{M_H}\xspace}
\def\Nl      {\ensuremath{M_L}\xspace}
\def\Nphys   {\ensuremath{\Nz_{phys}(t)}\xspace}
\def\Nbphys  {\ensuremath{\Nzb_{phys}(t)}\xspace}
\def\gh      {\ensuremath{\gamma_H}\xspace}
\def\gl      {\ensuremath{\gamma_L}\xspace}

\def\Bzd     {\ensuremath{B_d^0}\xspace}
\def\Bzs     {\ensuremath{B_s^0}\xspace}
\def\Bsd     {\ensuremath{B_{s(d)}^0}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bdpsikstar {\ensuremath{\Bd \to \jpsi \Kstarz}\xspace}
\def\bspsiphi   {\ensuremath{\Bs \to \jpsi \phi}\xspace}
\def\lblmumu    {\ensuremath{\Lambda_b \to \mup\mun \Lambda}\xspace}
\def\bsphimm    {\ensuremath{\Bs \to \phi\mup\mun}\xspace}
\def\bdkmm      {\ensuremath{\Bz \to K\mup\mun}\xspace}
\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bspsiphi   {\ensuremath{\Bs \to \jpsi \phi}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi \Kpm}\xspace}
\def\bupsimmk   {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosmm     {\ensuremath{b \to s \mup\mun}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}

\def\bbmumuX    {\ensuremath{\bbbar\to \mu^+\mu^-+X}\xspace}
\def\ccmumuX    {\ensuremath{\ccbar\to \mu^+\mu^-+X}\xspace}
\def\bpsimmX    {\ensuremath{b\to \jpsi(\to\mup\mun) X}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_\perp$}\xspace}
\def\ptrel      {\mbox{$p_\perp^{\mathrm{rel}}$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ke}{\ensuremath{\mbox{\,ke}}\xspace}

\newcommand{\eev}{\ensuremath{\mbox{\,Ee\kern -0.1em V}}\xspace}
\newcommand{\pev}{\ensuremath{\mbox{\,Pe\kern -0.1em V}}\xspace}
\newcommand{\tev}{\ensuremath{\mbox{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mbox{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mbox{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mbox{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev} {\ensuremath{\mbox{\,e\kern -0.1em V}}\xspace}
\def\microEv         {\ensuremath{\,\mu\mbox{eV}}\xspace}  %% micro eV
\def\milliEv     {\ensuremath{\,\mbox{meV}}\xspace}  %% micro eV
\newcommand{\gevc}{\ensuremath{{\mbox{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mbox{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mbox{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mbox{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\N   {\ensuremath{\mbox{\,N}\xspace}}


\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{\mbox{\,km}}\xspace}
\def\m    {\ensuremath{\mbox{\,m}}\xspace}
\def\cm   {\ensuremath{\mbox{\,cm}}\xspace}
\def\sr   {\ensuremath{\mbox{\,sr}}\xspace}
\def\cma  {\ensuremath{\mbox{\,cm}^2}\xspace}
\def\mm   {\ensuremath{\mbox{\,mm}\xspace}}
\def\mma  {\ensuremath{\mbox{\,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\mu\mbox{m}\xspace}}
\def\muma {\ensuremath{\,\mu\mbox{m^2}}\xspace}
\def\fm   {\ensuremath{\mbox{\,fm}}\xspace}
\def\nm   {\ensuremath{\mbox{\,nm}}\xspace}   %% nanometer
\def\nb   {\ensuremath{\mbox{\,nb}}\xspace}
%
\def\barn      {\ensuremath{\mbox{\,b}}\xspace}
\def\mbarn     {\ensuremath{\mbox{\,mb}}\xspace}
\def\mb        {\ensuremath{\mbox{\,mb}}\xspace}
\def\pb        {\ensuremath{\mbox{\,pb}}\xspace}
\def\invmb     {\ensuremath{\mbox{\,mb}^{-1}}\xspace}
\def\invnb     {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\invpb     {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\ub        {\ensuremath{\,\mu\mbox{b}}\xspace}
\def\invub     {\ensuremath{\mbox{\,\ub}^{-1}}\xspace}
\def\fb        {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb     {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab        {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab     {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\cms       {\ensuremath{\mbox{\,cm}^{-2}\mbox{s}^{-1}}\xspace}
\def\sqrts     {\ensuremath{\sqrt{s}}}


\def\mpc     {\ensuremath{\mbox{\,Mpc}}\xspace}

\def\kW   {\ensuremath{\mbox{\,kW}}\xspace}
\def\MW   {\ensuremath{\mbox{\,MW}}\xspace}
\def\mW   {\ensuremath{\mbox{\,mW}}\xspace}
\def\GW   {\ensuremath{\mbox{\,GW}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Hz  {\ensuremath{\mbox{\, Hz}}\xspace}
\def\kHz {\ensuremath{\mbox{\, kHz}}\xspace}
\def\MHz {\ensuremath{\mbox{\, MHz}}\xspace}


%\def\us   {\ensuremath{\mbox{\,\mu s}}\xspace}
\def\us   {\ensuremath{\,\mu\mbox{s}}\xspace}
\def\ns   {\ensuremath{\mbox{\,ns}}\xspace}
\def\ms   {\ensuremath{\mbox{\,ms}}\xspace}
\def\ps   {\ensuremath{\mbox{\,ps}}\xspace}
\def\fs   {\ensuremath{\mbox{\,fs}}\xspace}
\def\gm   {\ensuremath{\mbox{\,g}}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
%%?? kill NIM A ?? \def\year{\ensuremath{\mbox{\,y}}\xspace}
\def\Gy{\ensuremath{\mbox{\,Gy}}\xspace}
\def\sec{\ensuremath{\mbox{\,s}}\xspace}       %% second - this works - jw 4/19
\def\msec{\ensuremath{\mbox{\,ms}}\xspace}       %% second - this works - jw 4/19
\def\usec{\ensuremath{\,\mu \mbox{s}}\xspace}       %% second - this works - jw 4/19
\def\h          {\ensuremath{\mbox{\,h}\xspace}}

\def\kg         {\ensuremath{\mbox{\,kg}}\xspace}  %% kilogram
\def\gram       {\ensuremath{\mbox{\,g}}\xspace}  %% gram


\def\uTesla     {\ensuremath{\,\mu\mbox{T}}\xspace}  %% nanoTesla
\def\mTesla     {\ensuremath{\mbox{\,mT}}\xspace}  %% nanoTesla
\def\nTesla     {\ensuremath{\mbox{\,nT}}\xspace}  %% nanoTesla
\def\Tesla      {\ensuremath{\mbox{\,T}}\xspace}  %% Tesla
\def\Gauss      {\ensuremath{\mbox{\,G}}\xspace}  %% 

\def\mA     {\ensuremath{\mbox{\,mA}}\xspace}  %% mili Ampere
\def\Ampere     {\ensuremath{\mbox{\,A}}\xspace}  %% Ampere
\def\Amp     {\ensuremath{\mbox{\,A}}\xspace}  %% Ampere
\def\Watt     {\ensuremath{\mbox{\,W}}\xspace}  %% Ampere

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\mbar        {\ensuremath{\mbox{\,mbar}}}   %% milibar

%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\MVolts {\ensuremath{\mbox{\, MV}}\xspace}
\def\kVolts {\ensuremath{\mbox{\, kV}}\xspace}
\def\Volts {\ensuremath{\mbox{\, V}}\xspace}
\def\Volt  {\ensuremath{\mbox{\, V}}\xspace}
\def\atm   {\ensuremath{\mbox{\,atm}}\xspace}
\def\Ke    {\ensuremath{\mbox{\, K}}\xspace}
\def\mKe   {\ensuremath{\mbox{\, mK}}\xspace}
\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath{\mbox{K}}\xspace}
\def\degrees {\ensuremath{^{\circ}}\xspace}
\def\mrad {\ensuremath{\,\mbox{mrad}}\xspace}               %% milliradian
\def\urad {\ensuremath{\,\mu\mbox{rad}}\xspace}               %% milliradian
\def\rad{\ensuremath{\mbox{\,rad}}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\sstat}{\ensuremath{\sigma_{\mathrm{stat}}}\xspace}
\newcommand{\ssyst}{\ensuremath{\sigma_{\mathrm{syst}}}\xspace}

\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%


% -- SUSY
\def\tb         {\ensuremath{\tan\beta}\xspace}



% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\asp}{\ensuremath{{\alpha_{\scriptscriptstyle S}\over\pi}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!

\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instr.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseC~A~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\delphes    {\mbox{\tt Delphes}\xspace}
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\sherpa     {\mbox{\tt Sherpa}\xspace}
\def\pythia     {\mbox{\tt Pythia}\xspace}
\def\powheg     {\mbox{\tt Powheg}\xspace}
\def\mcatnlo    {\mbox{\tt MC@NLO}\xspace}
\def\hpp        {\mbox{\tt Herwig++}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}

\def\hdecay     {\mbox{\tt Hdecay}\xspace}
\def\prophecy4f {\mbox{\tt Prophecy4f}\xspace}

